LightDP: Towards Automating Differential Privacy Proofs

The growing popularity and adoption of differential privacy in academic and industrial settings has resulted in the development of increasingly sophisticated algorithms for releasing information while preserving privacy. Accompanying this phenomenon is the natural rise in the development and publication of incorrect algorithms, thus demonstrating the necessity of formal verification tools. However, existing formal methods for differential privacy face a dilemma: methods based on customized logics can verify sophisticated algorithms but come with a steep learning curve and significant annotation burden on the programmers, while existing programming platforms lack expressive power for some sophisticated algorithms. In this paper, we present LightDP, a simple imperative language that strikes a better balance between expressive power and usability. The core of LightDP is a novel relational type system that separates relational reasoning from privacy budget calculations. With dependent types, the type system is powerful enough to verify sophisticated algorithms where the composition theorem falls short. In addition, the inference engine of LightDP infers most of the proof details, and even searches for the proof with minimal privacy cost bound when multiple proofs exist. We show that LightDP verifies sophisticated algorithms with little manual effort.

==> commondefs <==
#
# See the manual page for "commondefs" for more information.
#

INCLDIR = $(ROOT)/usr/include
TEXDIR = ../tex-macros

COMMONRULES = $(MAKEDIR)/commonrules

SOURCES = $(CFILES) $(C++FILES) $(YFILES) $(LFILES) $(AFILES)
OBJECTS = $(CFILES:.c=.o) $(C++FILES:.C=.o)
DIRT = *.o core *.aux *.dvi *.log *.stamp *.i *.bbl *.[ib]lg $(LDIRT)
GENERATED = .dependtime Makedepend Makedepend.bak
RM = rm -f
MKDEPFILE = Makedepend
MKDEPEND = makedepend
MKDEPFLAGS = -Y
MKDEPC++FLAGS = $(C++DEFS) $(C++INCS) $(MKDEPFLAGS)
MKDEPCFLAGS = $(CDEFS) $(CINCS) $(MKDEPFLAGS)

.SUFFIXES: .C .ps .i .txt .h
.SUFFIXES: .tex .dvi .ind .idx .bbl .aux .glo .aux .stamp .pdf .eps

GNUBIN = /usr/local

ATTC++ = CC
DECC++ = cxx
GNUC++ = g++

CC = cc
C++ = $(GNUC++)
YACC = bison
DVIPS = dvips

C++F = $(C++) $(C++FLAGS)
CCF = $(CC) $(CFLAGS)

C++FLAGS = $(C++OPTS) $(C++DEFS) $(C++INCS)

C++INCS = $(GC++INCS) $(LC++INCS)
C++OPTS = $(GC++OPTS) $(LC++OPTS)
C++DEFS = $(GC++DEFS) $(LC++DEFS)

GC++OPTS = $(OPTIMIZER)

CFLAGS = $(COPTS) $(CDEFS) $(CINCS)
COPTS = $(GCOPTS) $(LCOPTS)
CDEFS = $(GCDEFS) $(LCDEFS)
CINCS = $(GCINCS) $(LCINCS)

GCOPTS = $(OPTIMIZER)

M3F = $(M3) $(M3FLAGS)
M3 = m3
M3PP = m3pp

LDFLAGS = $(LLDFLAGS) $(GLDFLAGS)
LLDFLAGS = $(LLDLIBS) $(LLDOPTS) 

SEP=:
#SEP=\;         # for MikTeX+Cygwin
TEXINPUTS = .$(SEP)$(TEXDIR)$(SEP)
LATEX = TEXINPUTS='$(TEXINPUTS)' latex --output-directory='$(BUILD)'
PDFLATEX = TEXINPUTS='$(TEXINPUTS)' pdflatex --output-directory='$(BUILD)'
BIBTEX = bibtex

# Directory for TeX's generated files.
BUILD = .
# BUILDD should be equivalent to $(BUILD)/
BUILDD =
VPATH = $(BUILD)

-include localdefs


==> commonrules <==
# Some basic recursive rules for building, installing, and cleaning up
# a source tree
#
subdirs:
	@sub="$(SUBDIRS)"; \
	for i in $$sub; do if test -n "$$i"; then \
	      (cd $$i; make); \
	fi; done;

clean:  localclean
	@sub="$(SUBDIRS)"; \
	for i in $$sub; do if test -n "$$i"; then \
	      (cd $$i; make $@); \
	fi; done;

localclean:
	$(RM) $(DIRT)

clobber: localclean
	@sub="$(SUBDIRS)";						      \
	for i in $$sub; do if test -n "$$i"; then			      \
	      (cd $$i; make $@);					      \
	fi; done;
	$(RM) $(TARGETS) $(GENERATED)

install: default localinstall
	@sub="$(SUBDIRS)";						      \
	for i in $$sub; do if test -n "$$i"; then			      \
	      (cd $$i; make $@);					      \
	fi; done;

incdepend: .dependtime
depend: .dependtime

.dependtime: $(SOURCES)
	touch temp
	$(MKDEPEND) $(MKDEPC++FLAGS) -f temp $(C++FILES)
	touch $(MKDEPFILE)
	$(MKDEPEND) $(MKDEPCFLAGS) -f $(MKDEPFILE) $(CFILES)
	cat temp >> $(MKDEPFILE)
	$(RM) temp
	touch $@

# Rules for TeX files
#
# The line that runs LATEX needs to run inside a subshell to turn off
# "make"'s status checking. It blows away .aux because the .aux file
# created is bad and also breaks bibtex. It touches .stamp to force a
# rebuild.
.tex.dvi:
	@if test -r "$*.aux";						      \
	   then cp "$(BUILDD)$*.aux" "$(BUILDD)$*.auxprev";		      \
	   else echo > "$(BUILDD)$*.auxprev";				      \
	fi
	@echo "$(LATEX) $<"
	@sh -c "$(LATEX) $< || ($(RM) $*.aux; sleep 1; touch \"$(BUILDD)$*.stamp\"; exit 1)"
	@-cmp -s "$(BUILDD)$*.aux" "$(BUILDD)$*.auxprev";		      \
	if test $$? = 1;						      \
	then								      \
	    sleep 1;							      \
	    echo "==> Rebuilding $@";					      \
	    touch "$(BUILDD)$*.stamp";					      \
	    $(MAKE) $@;							      \
	else								      \
	    echo "==> No need to rebuild $@";				      \
	fi
	@$(RM) "$(BUILDD)$*.auxprev"

.tex.pdf:
	@if test -r "$(BUILDD)$*.aux";					      \
	   then cp "$(BUILDD)$*.aux" "$(BUILDD)$*.auxprev";		      \
	   else echo > "$(BUILDD)$*.auxprev";				      \
	fi
	@echo "$(PDFLATEX) $<"
	@sh -c "$(PDFLATEX) $< || ($(RM) $*.aux; sleep 1; touch \"$(BUILDD)$*.stamp\"; exit 1)"
	@-cmp -s "$(BUILDD)$*.aux" "$(BUILDD)$*.auxprev";		      \
	if test $$? = 1;						      \
	then								      \
	    sleep 1;							      \
	    echo "==> Rebuilding $@";					      \
	    touch "$(BUILDD)$*.stamp";					      \
	    $(MAKE) $@;							      \
	else								      \
	    echo "==> No need to rebuild $@";				      \
	fi
	@$(RM) "$(BUILDD)$*.auxprev"

# must add dependencies like
#    foo.ind: foo.stamp
#    foo.dvi: foo.ind
# to use this rule properly.
.tex.ind:
	@if [ -f $*.idx ]; then						      \
	   echo makeindex $*.idx;					      \
	   makeindex $*.idx;						      \
	else								      \
	   echo touch $@;						      \
	   touch $@;							      \
        fi

# must add dependencies like
#    foo.bbl: foo.bib
#    foo.dvi: foo.bbl
# to use this rule properly.
.tex.bbl:
	@if [ -r $*.aux ]; then echo $(BIBTEX) $*; sh -c "$(BIBTEX) $* || echo"; else echo; fi

.tex.stamp: # backward compatibility
	touch $@

.dvi.ps:
	$(DVIPS) $(DVIPSOPTS) $< -o $@
.eps.pdf:
	epstopdf $(EPSTOPDFOPTS) $<

#
# Rules for C++ and .i files
#

.C.i:
	$(C++F) -E $< > $@

.c.i:
	$(CCF) -E $< > $@

.C.o:
	$(C++F) -c $<

# include $(M3SU)    # old Modula-3 rules

